ViViT: A Video Vision Transformer

We present pure-transformer based models for video classification, drawing upon the recent success of such models in image classification. Our model extracts spatio-temporal tokens from the input video, which are then encoded by a series of transformer layers. In order to handle the long sequences of tokens encountered in video, we propose several, efficient variants of our model which factorise the spatial- and temporal-dimensions of the input. Although transformer-based models are known to only be effective when large training datasets are available, we show how we can effectively regularise the model during training and leverage pretrained image models to be able to train on comparatively small datasets. We conduct thorough ablation studies, and achieve state-of-the-art results on multiple video classification benchmarks including Kinetics 400 and 600, Epic Kitchens, Something-Something v2 and Moments in Time, outperforming prior methods based on deep 3D convolutional networks. To facilitate further research, we release code at https://github.com/google-research/scenic/tree/main/scenic/projects/vivit

==> figures/ablation/views_accuracy.tex <==
\begin{figure}[tb]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/ablation/views_accuracy_fig.pdf}
	\caption{
		The effect of varying the number of frames input to the network when keeping the number of tokens constant by adjusting the tubelet length $t$. We use ViViT-B, and spatio-temporal attention on Kinetics 400.
		A Kinetics video contains 250 frames (10 seconds sampled at 25 fps) and the accuracy for each model saturates once the number of equidistant temporal views is sufficient to ``see'' the whole video clip.
	}
	\label{fig:ablation_views_acc}
	\vspace{-\baselineskip}
\end{figure}

==> figures/kinetics_accuracy_flops.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/kinetics_accuracy_flops_fig.pdf}
        \caption{ 
    	Top-1 accuracy vs FLOPs on Kinetics 400, as the number of views is varied.
    	Our models achieve Pareto-optimal points as they require fewer views to obtain high accuracy compared to SlowFast~\cite{feichtenhofer_iccv_2019} and X3D~\cite{feichtenhofer_cvpr_2020}.
    	Data for \cite{feichtenhofer_iccv_2019,feichtenhofer_cvpr_2020} from Fig.~3 of~\cite{feichtenhofer_cvpr_2020}.
    }
    \label{fig:kinetics_acc_flops}
\end{figure}
